YouTube-8M: A Large-Scale Video Classification Benchmark

Many recent advancements in Computer Vision are attributed to large datasets. Open-source software packages for Machine Learning and inexpensive commodity hardware have reduced the barrier of entry for exploring novel approaches at scale. It is possible to train models over millions of examples within a few days. Although large-scale datasets exist for image understanding, such as ImageNet, there are no comparable size video classification datasets. In this paper, we introduce YouTube-8M, the largest multi-label video classification dataset, composed of ~8 million videos (500K hours of video), annotated with a vocabulary of 4800 visual entities. To get the videos and their labels, we used a YouTube video annotation system, which labels videos with their main topics. While the labels are machine-generated, they have high-precision and are derived from a variety of human-based signals including metadata and query click signals. We filtered the video labels (Knowledge Graph entities) using both automated and manual curation strategies, including asking human raters if the labels are visually recognizable. Then, we decoded each video at one-frame-per-second, and used a Deep CNN pre-trained on ImageNet to extract the hidden representation immediately prior to the classification layer. Finally, we compressed the frame features and make both the features and video-level labels available for download. We trained various (modest) classification models on the dataset, evaluated them using popular evaluation metrics, and report them as baselines. Despite the size of the dataset, some of our models train to convergence in less than a day on a single machine using TensorFlow. We plan to release code for training a TensorFlow model and for computing metrics.

==> fisher-vlad.tex <==
\subsection{Fisher Vectors and VLAD}
For the task of aggregating local descriptors into compact fixed-length representations, Fisher Vectors~\cite{fisher1} and VLAD~\cite{vlad} are a powerful
class of encoding schemes that have traditionally provided some of the best results for both image understanding~\cite{fisher1,fisher2,vlad} and
action/video understanding~\cite{fisher-action, vlad-action}. The Fisher Vector (FV) and VLAD representations can be seen as extensions of the popular
 bag-of-visual-words (BOW) representation~\cite{bow}. While all three representations are based on a dictionary of the local descriptors, the FV representation
explicitly encodes the gradients of the log likelihood of the probability density function (using Gaussian Mixture Models) of the descriptors while the
VLAD characterizes the distribution of the local descriptors with respect to the dictionary centers. Empirically, the FV and VLAD representations have been
shown to improve over the BoW representation by providing second-order information about the distribution of local descriptors.

\subsubsection{Fisher Vectors}
\label{sec:fisher}
Assuming that the input frame-level features $\{x_t \in \mathbb{R}^D, t = 1 ... T\}$ of a video $V$ are generated independently by a Gaussian mixture model
 (GMM) with $k$ components and a diagonal co-variance matrix, the Fisher vector representation is obtained by concatenating the gradients of the Fisher Kernel with
 respect to the mean and standard deviation parameters. Let $\lambda = \{w_i, \mu_i, \Sigma_i, i = 1...N\}$ be the parameters of the GMM where $w_i$, $\mu_i$ and
$\Sigma_i$ denote respectively the weight, mean vector and covariance matrix, and $N$ is the number of mixtures. And let $\gamma_i(x_t)$ denote the probability
that the descriptor $x_t$ is assigned to Gaussian $i$. Then the normalized gradient with respect to the mean and standard deviation is given by
(see also~\cite{fisher2}),

\begin{eqnarray}
  \tau_{\mu_i} (V) &=& \frac{1}{T \sqrt{w_i}} \sum_{t = 1}^{T} \gamma_i(x_t) \left(\frac{x_t - \mu_i}{\sigma_i}\right), \label{eq:fisher1} \\
  \tau_{\sigma_i} (V) &=& \frac{1}{T \sqrt{2w_i}} \sum_{t = 1}^{T} \gamma_i(x_t) \left[\frac{(x_t - \mu_i)^2}{(\sigma_i)^2} - 1\right]. \label{eq:fisher2}
\end{eqnarray}

The final representation is obtained by concatenating the gradients in Equations~\eqref{eq:fisher1} and \eqref{eq:fisher2} for all the gaussians $i = 1...N$. Hence the final
dimensionality of the FV representation is $2ND$ where $N$ is the number of mixtures and $D$ is the dimension of the input vectors. In many cases an initial PCA is performed on the input vectors in order to reduce the overall dimensionality. We used in our experiments $N = \{4, 8, 16\}$ and reduced dimensionality with PCA to $\{128, 256, 512, 1024\}$.

\subsubsection{VLAD}
\label{sec:vlad}
The VLAD descriptor can be seen as a simplification of the FV representation. Instead of a GMM, the dictionary $\mathbb{C} = \{c_1,...c_k\}$ of size $k$ of the
local descriptors is obtained by clustering a sample of the descriptors using $k$-means. Each input frame-level feature $x_t$ is then associated to its nearest
dictionary vectors $c_i = NN(x_t)$. The VLAD descriptor is then obtained by accumulating, for each dictionary vector $c_i$, the differences $x_t - c_i$ of the
vectors $x_t$ assigned to $c_i$. Each individual accumulated difference is $L_2$ normalized. The final aggregated vector is again $L_2$-normalized to obtain the final VLAD descriptor whose dimensionality is therefore
 $kD$. See~\cite{vlad} for more details.
 Similar to the FV representation, dimensionality reduction of the input features is performed using PCA in order to utilize more clusters and reduce the overall dimensionality. Similarly to FV, we used $k = \{4, 8, 16\}$, and PCA dimensions out of $\{128, 256, 512, 1024\}$.


==> mixture-of-experts-online.tex <==
\subsection{Mixture of Experts}
%
Mixture of experts (MoE) was first proposed by Jacobs and Jordan~\cite{Jordan94hierarchicalmixtures}. In an MoE model, each individual component models a different binary probability distribution. The probability of choosing the expert is modeled as another probability distribution. We use the following probability distribution of the label given the features:
\begin{equation}
p(y = 1 | \mathbf{x}) = \sum_{h} p(h | \mathbf{x}) p(y = 1 | \mathbf{x}, h),
\end{equation}
where the conditional probability of the hidden state given the features is a soft-max over $H+1$ states, that is,
\begin{equation}
p(h | \mathbf{x}) = \frac{\exp(\mathbf{w}_h^{T} \mathbf{x})}{1 + \sum_{h'} \exp(\mathbf{w}_{h'}^{T} \mathbf{x})}.
\end{equation}
The last, $(H+1)^{th}$, state is a dummy state that always results in the non-existence of the entity. The conditional probability of $y=1$ given the hidden state and the features is a logistic regression given as $p(y = 1 | \mathbf{x}, h) = \sigma(\mathbf{u}_h^{T} \mathbf{x})$.
When $H=1$, it is a product of two logistics, and hence it is more general than logistic regression. The parameters to estimate are the softmax gating weights $\mathbf{w}_h$ for each hidden state and the expert logistic weights $\mathbf{u}_h$. For the sake of brevity, we will denote $p_{y|\mathbf{x}} = p(y=1 | \mathbf{x})$, $p_{h|\mathbf{x}} = p(h | \mathbf{x})$ and $p_{h} = p(y=1 | \mathbf{x},h)$. Given a set of training data ${(\mathbf{x}_i, g_i)}_{i=1\ldots N}$ for each label, where $\mathbf{x}_i$ is the feature vector and $g_i$ is the corresponding boolean ground-truth, we optimize the regularized loss of the data:
\begin{equation}
\sum_{i=1}^{N}  w_i \mathcal{L} \left[p_{y|\mathbf{x}_i}, g_t\right] +\lambda_{2} \left(\Vert \mathbf{w} \Vert_{2}^2 + \Vert \mathbf{u} \Vert_{2}^2 \right),
\label{eqn:loss}
\end{equation}
where $\mathcal{L}(p,g) = -g \log p - (1-g) \log (1-p)$ is the log-loss and $w_i$ is the weight for the $i^{th}$ example.

\subsubsection{Optimization}
We could directly write the derivative of $\mathcal{L} \left[p_{y|\mathbf{x}}, g\right]$ with respect to the softmax weight $\mathbf{w}_h$ and the logistic weight $\mathbf{u}_h$ as
\begin{eqnarray*}
\frac{\partial \mathcal{L} \left[p_{y|\mathbf{x}}, g\right]}{\partial \mathbf{w}_h} &=& \mathbf{x} \frac{p_{h|\mathbf{x}} \left(p_{y|h,\mathbf{x}} - p_{y|\mathbf{x}}\right) \left(p_{y|\mathbf{x}}-g\right)}{p_{y|\mathbf{x}}(1-p_{y|\mathbf{x}})} \\
\frac{\partial \mathcal{L} \left[p_{y|\mathbf{x}}, g\right]}{\partial \mathbf{u}_h} &=& \mathbf{x} \frac{p_{h|\mathbf{x}} p_{y|h,\mathbf{x}} (1- p_{y|h,\mathbf{x}})\left(p_{y|\mathbf{x}}-g\right)}{p_{y|\mathbf{x}}(1-p_{y|\mathbf{x}})}
\end{eqnarray*}


\subsection{Online training}

Our training data consists of about 7M videos. For our frame level models, we have about 1 billion training examples (multiple frames sampled across multiple videos). To deal with such a large scale training data, we implemented an online training version of the MoE model that consists of the following steps:
\newline
\noindent
\textbf{Sampling: } Randomly sample \textbf{up to} M positives and M negatives in each iteration. We use $M=200,000$.\footnote{Note that the choice of $M$ only affects the convergence and not the final results.}
\newline
\noindent
\textbf{Preserving the distribution:} Assuming that $S_p$ positives and $S_n$ negatives have been sampled of the $T_p$ true positives and $T_n$ true negatives, we re-weight the positives and negatives using scales $w_{+}$ and $w_{-}$ such that $\frac{w_{+} S_p}{w_{-} S_n} = \frac{T_p}{T_n}$. To avoid too much deviation between $w_{+}$ and $w_{-}$, we set $w_+ = \frac{1}{w_-} = \sqrt{\frac{T_p S_n}{T_n S_p}}$.
\newline
\noindent
\textbf{Adagrad:} In each iteration, we use Adagrad to update the model for each label from the collected samples. We use a mini batch size of 1 and an L2-weight of $10^{-6}$ for our experiments. Since each label is treated independently, multiple machines are used to process the various labels in parallel.
\newline
\noindent
\textbf{Feature preprocessing: } The dense feature vectors, which have already undergone a PCA transformation and whitening, are further processed with L2-normalization. The full preprocessing formula starting from the RELU outputs of a deep image annotation model is given by $\mathbf{z} = \frac{\mathbf{A} (\mathbf{x} - \mathbf{\mu})}{\Vert \mathbf{A} (\mathbf{x} - \mathbf{\mu}) \Vert_{2}}$. The L2-normalization procedure ensures the gradients are well behaved by preventing outliers from introducing very high gradient values. We do not do this normalization when dealing with sparse features.


